Higher-order probabilistic adversarial computations: Categorical semantics and program logics

Adversarial computations are a widely studied class of computations where resource-bounded probabilistic adversaries have access to oracles, i.e., probabilistic procedures with private state. These computations arise routinely in several domains, including security, privacy and machine learning. In this paper, we develop program logics for reasoning about adversarial computations in a higher-order setting. Our logics are built on top of a simply typed $\lambda$-calculus extended with a graded monad for probabilities and state. The grading is used to model and restrict the memory footprint and the cost (in terms of oracle calls) of computations. Under this view, an adversary is a higher-order expression that expects as arguments the code of its oracles. We develop unary program logics for reasoning about error probabilities and expected values, and a relational logic for reasoning about coupling-based properties. All logics feature rules for adversarial computations, and yield guarantees that are valid for all adversaries that satisfy a fixed resource policy. We prove the soundness of the logics in the category of quasi-Borel spaces, using a general notion of graded predicate liftings, and we use logical relations over graded predicate liftings to establish the soundness of proof rules for adversaries. We illustrate the working of our logics with simple but illustrative examples.

==> adversaries.tex <==
\section{Adversarial properties}\label{sec:adv}

In this section we finally introduce the notion of adversary, and the
rules to reason about them.

Security properties are often expressed in an adversarial setting. Instead of
specifying how a program behaves with respect to its input, we specify how this
program must behave when interacting with another unknown and arbitrary program
(the adversary).  Since its code is unknown, we cannot use our syntax-directed
logic directly to reason about this program, and we need to develop specialised
rules. We distinguish two possible settings
\begin{itemize}
    \item {\bf Manager adversary}. Here, the adversary is a computation of
        at least second order. It receives as an input a probabilistic
        program $\cO \colon \sigma \to \sfT(\tau)$, called the oracle. The
        type of the adversary after erasing state gradings \sk{There is nothing like a state erasure at syntactic level because every $\sfT$ type must take $\Sigma,k$.}
        is $\cA \colon (\sigma\to\sfT(\tau))\to\sfT(\tau')$.
        They have some shared memory, although the oracle may have its own
        private memory. The oracle is limited in the number of times it can
        call the oracle. This is the way the security of many cryptographic protocols
        is stated.

    \item {\bf Worker adversary}. Here, the adversary is a computation of the
        same erased type as the oracle(s), $\cO,\cA \colon \sigma \to
        \sfT(\tau)$.  They possibly have some shared memory, and each
        computation may have their own private memory. There is some known
        higher-level procedure that calls and coordinates the oracles and adversaries.
        This is the case for instance of multiparty computation with malicious
        participants. Here we can distinguish between adversaries that have
        access to the other participants and adversaries that do not.
\end{itemize}

The general idea is that type of the adversaries is going to be annotated
with the memory locations it can access, and this guarantees a property
that the adversary must satisfy. For instance, and adversary of type
$\sigma \to \sfT_{\Sigma}(\tau)$ preserves any property $\phi$ on the memory
that does not depend on $\Sigma$. \sk{No $k$ annotated here.} This is captured by the rule \rname{W-ADV-U}
in Figure~\ref{fig:adv-rules}. The independence of $\phi$ from $\Sigma$ is
captured by the following notion of safety:

\begin{definition}
    Let $\phi$ be a predicate on memories and $\Sigma \subseteq \loc$. We say
    that $\phi \in {\sf Safe}(\Sigma)$ if and only if,
\[ \forall m. \forall l \in \Sigma. \forall v \in \tval. 
    \phi(m)  \Rightarrow \phi(m[l\mapsto v])
\]

\end{definition}


\aag{It may be clearer to have instead the notation $l \in {\sf Safe}(\phi)$
    meaning ``writing in location $l$ preserves $\phi$'', and then
    have the condition $\Sigma \subseteq {\sf Safe}(\phi)$
}

As an example, let $\phi \equiv \st[a]=\st[b]$ for some $a,b\in\loc$.
Then, for all $\Sigma$ such that $a,b \not\in \Sigma$ we have
that $\phi \in \safe{\Sigma}$.

The more interesting case is the case of adversaries that have access to
oracles. Here we can restrict not only the memory locations the adversary
can access directly (rather than through the oracle), but also the number
of times the oracle can be called.
$\cA(\cO)$ preserves $\phi$ (called \emph{the invariant}). 
%
%In HO-UBL, adversarial
%properties can be expressed (omitting gradings) as:
%\begin{equation}
%\label{eq:adv-property}
%    \cA \colon (\sigma \to \cT(\tau)) \to \cT(\tau') \vdash
%    \{ \phi \}    
%~\cA(\cO) \colon \cT(\tau')~
%\{\!\{ \phi \}\!\}
%\end{equation}
%Here $\cA$ is a variable, but $\cO$ stands for a concrete term with a known
%syntax, from which we assume:
%\[ \vdash \{\phi\}~\cO \colon \sigma\to\cT(\tau)~\{\!\{\phi\}\!\} \]
%In general, it is not possible to prove~(\ref{eq:adv-property}) with any further
%assumption. If there is no memory separation between $\cO$ and $\cA$,
%then $\cA$ could conceivably break the invariant. This memory separation
%can be enforced by restricting the syntax of $\cA$ to not access any
%location that $\cO$ accesses, but a more principled alternative is
%to restrict it by properly annotating the type of $\cA$.
%
Assume the adversary has type:
\[
    \cA :\forall \alpha. (\sigma \to \mon{\alpha,1}{\tau}) 
        \to \mon{\Sigma \cup \alpha, k}{\tau'}
\]
This states that the oracle has a private memory region that is abstracted by
$\alpha$ and that the memory footprint of the whole computation is
$\alpha\cup\Sigma$. Since the memory footprint of the adversary cannot depend
on $\alpha$, then it must be that the memory region that the adversary accesses
directly is restricted to $\Sigma$.  In addition, the type states that the
adversary can call the oracle up to $k$ times. 
%
If we now set an invariant $\phi$ that does not depend on $\Sigma$ then the
adversary should not be able to break $\phi$. The rule \rname{M-ADV} on
Figure~\ref{fig:adv-rules} can be used to reason in this setting.
What this rule states is that if
\begin{enumerate}
    \item $\phi$ is an invariant safe for $\Sigma$,
    \item $\cO$ is an oracle that preserves $\phi$ at least with probability $1-\delta$, and
    \item $\cA$ is an arbitrary adversary that only writes to $\Sigma$ and that
        can call $\cO$ up to $k$ times,
\end{enumerate}
then $\cA(\cO)$ will preserve $\phi$ at least with probability $1-\delta$

For simplicity we present the rule in an empty context and assuming
$\sigma,\tau$ and $\tau'$ are non-monadic. These restrictions can be
lifted by adding extra logical premises.



\begin{figure}
\begin{gather*}
\inferrule*[right= \sf M-ADV-U]
{\cdot \vdash \cA :\forall \alpha. (\sigma \to \mon{\alpha,1}{\tau}) \to \mon{\Sigma \cup \alpha, k}{\tau'} \\
    \aumj{ x : \sigma}{\Psi}{\phi}{t}{\mon{\Sigma',1}{\tau}}{\phi}{\delta} \\
    \holwf{\st:M}{\phi} \\
 \phi \in {\sf Safe}(\Sigma) \\
 \sigma,\tau,\tau'\ \text{non-monadic types}
}
{\aumj{\cdot}{\Psi}{\phi}{\cA(\lambda x. t)}{\mon{\Sigma\cup\Sigma',k}{\tau}}{\phi}{k\cdot\delta}}
\\
\inferrule*[right = \sf W-ADV-U]
{\cdot \vdash \cA : \sigma \to \mon{\Sigma, k}{\tau'} \\
    \holwf{\st:M}{\phi} \\
 \phi \in {\sf Safe}(\Sigma) \\
 \sigma,\tau,\tau'\ \text{non-monadic types}
}
{\aumj{\cdot}{\Psi}{\phi}{\cA(\lambda x. t)}{\mon{\Sigma,k}{\tau}}{\phi}{0}}
\end{gather*}
\caption{Adversary rules}
\label{fig:adv-rules}
\end{figure}




==> base-logic.tex <==
\section{Preliminaries: Higher-Order Program Logics}\label{sec:logics}

In this section, we briefly review the syntax and semantics of
Higher-Order Logic and its unary and relational variants. These logics
were introduced in~\cite{ABGGS17}, and given a $\QBS$ semantics
in~\cite{SatoABGGH19}. Later, we shall use these logics for reasoning
about non-monadic computations. In this section we omit the concrete
derivation rules, which can be found either in \textit{op. cit.} or
in the full version of this paper.\gb{say the logic is  defined on
  non-monadic expressions}

\subsection{HOL}

Our base logic is HOL, a logic over higher-order programs.  The syntax
of our formulas is given below, where $R$ ranges over base predicates
and $\sigma$ ranges over types in the language:
\[
\phi, \psi ::= R(e_1, \dots, e_n) \mid \phi \wedge \psi \mid \phi \vee \psi \mid 
 \neg \phi \mid \phi \Rightarrow \psi \mid \forall x : \sigma. \phi \mid
  \exists x:\sigma. \phi.
\]

Well-formedness of a predicate $\phi$ in a typing context $\Gamma$ is denoted 
$\holwf{\Gamma}{\phi}$.
%, and the rules are defined in Figure~\ref{fig:hol-wf}.

Judgements in HOL are of the form $\jhol{\Gamma}{\Psi}{\phi}$, with
the intuitive meaning that $\phi$ is a well-formed formula under a
typing context $\Gamma$ that can be inferred from the set of premises
$\Psi$, each of which is also well-formed under $\Gamma$.  A selection
of rules for HOL is presented in Figure~\ref{fig:hol}.\gb{put the
  rules in appendix}
  \tetsuya{Put the rules in appendix.}
  
\begin{toappendix}
\begin{figure}
\small
\begin{gather*}
    \inferrule*{R \subseteq t_1 : \tau_1 \times\dots\times t_k : \tau_k \\
    \Gamma \vdash t_1 : \tau_1 \dots \Gamma \vdash t_k : \tau_k}
    {\holwf{\Gamma}{R(t_1,\dots,t_k)}}
    \qquad
    \inferrule*{\holwf{\Gamma}{\phi_1}\\ \holwf{\Gamma}{\phi_2}}
        {\holwf{\Gamma}{\phi_1 \wedge \phi_2}}
    \qquad
    \inferrule*{\holwf{\Gamma}{\phi_1}\\ \holwf{\Gamma}{\phi_2}}
        {\holwf{\Gamma}{\phi_1 \To \phi_2}}
    \\
    \inferrule*{\holwf{\Gamma, x : \tau}{\phi}}
        {\holwf{\Gamma}{\forall x. \phi}}
    \qquad
    \inferrule*{\holwf{\Gamma, x : \tau}{\phi}}
        {\holwf{\Gamma}{\exists x. \phi}}
\end{gather*}
\caption{Selected well-formedness rules of HOL}\label{fig:hol-wf}
\end{figure}

\begin{figure}
\small
\begin{gather*}
    \inferrule*[Right = Ax]
    {}
    {\jhol{\Gamma}{\Psi,\phi}{\phi}}
    \qquad
    \inferrule*[Right = $\land_I$]
    {\jhol{\Gamma}{\Psi}{\phi_1}\\ \jhol{\Gamma}{\Psi}{\phi_2}}
    {\jhol{\Gamma}{\Psi}{\phi_1 \wedge \phi_2}} \\
\qquad
    \inferrule*[Right = $\land_E$]{\jhol{\Gamma}{\Psi}{\phi_1 \wedge \phi_2}}
    {\jhol{\Gamma}{\Psi}{\phi_1}}
\qquad
    \inferrule*[Right = $\To_I$]
    {\jhol{\Gamma}{\Psi, \phi_1}{\phi_2}}
    {\jhol{\Gamma}{\Psi}{\phi_1 \To \phi_2}} \\
\qquad
    \inferrule*[Right = $\To_E$]
    {\jhol{\Gamma}{\Psi}{\phi_1 \To \phi_2} \\
    \jhol{\Gamma}{\Psi}{\phi_1}}
    {\jhol{\Gamma}{\Psi}{\phi_2}}
\end{gather*}
\caption{Selected HOL rules}\label{fig:hol}
\end{figure}
\end{toappendix}

\subsection{UHOL}

Starting from the base logic, we develop a unary program logic that we
call UHOL for unary higher-order logic.  This logic has non-monadic
judgments of the form $\juhol{\Gamma}{\Psi}{t}{\sigma}{\phi}$, which
combine a typing judgment $\Gamma\vdash t :\sigma$ and a logical
judgment $\jhol{\Gamma}{\Psi}{\phi[t/\res]}$. Here, $\res : \sigma$ is
a distinguished variable that appears free in $\phi$ to denote the
value of $t$, and $\Gamma, \res : \sigma\vdash \phi$, i.e.\, $\phi$ is
a valid assertion in context $\Gamma, \res : \sigma$. The rules of
UHOL are directed by the syntax of $t$. A selection of UHOL rules for
this fragment appears in Figure~\ref{fig:uhol}.\gb{put the rules in appendix}
\tetsuya{Put the rules in appendix.}

\begin{toappendix}
\begin{figure*}
\small
\begin{gather*}
\inferrule*[right = \sf U-VAR]
 {\jlc{\Gamma}{x}{\sigma} \\ \jhol{\Gamma}{\Psi}{\phi\subst{\res}{x}}}
 {\juhol{\Gamma}{\Psi}{x}{\sigma}{\phi}}
\qquad
\inferrule*[right= \sf U-ABS]
  {\juhol{\Gamma,x:\tau}{\Psi,\phi'}{t}{\sigma}{\phi}}
  {\juhol{\Gamma}{\Psi}{\lambda x:\tau. t}{\tau \to \sigma}{\forall x. \phi'
    \Rightarrow \phi\subst{\res}{\res\ x}}}
\\
\inferrule*[right= \sf U-APP]
      {\juhol{\Gamma}{\Psi}{t}{\tau\to \sigma}{\forall x.
        \phi'\subst{\res}{x}\Rightarrow\phi\subst{\res}{\res\ x}}\\ \juhol{\Gamma}{\Psi}{u}{\tau}{\phi'}}
  {\juhol{\Gamma}{\Psi}{t\ u}{\sigma}{\phi\subst{x}{u}}}
  \\
\inferrule*[right = \sf U-SUB]
    {\juhol{\Gamma}{\Psi}{t}{\sigma}{\phi'} \\
           \jhol{\Gamma}{\Psi}{\phi'\subst{\res}{t} \Rightarrow \phi\subst{\res}{t}}}
    {\juhol{\Gamma}{\Psi}{t}{\sigma}{\phi}}
    \\
\inferrule*[right= \sf U-CASE]
{\juhol{\Gamma}{\Psi}{t}{\sigma}{b \Rightarrow \phi} \\
\juhol{\Gamma}{\Psi}{u}{\sigma}{\neg b \Rightarrow \phi}}
        {\juhol{\Gamma}{\Psi}{\casebool{b}{t}{u}}{\sigma}{\phi}}
\end{gather*}
\caption{Selected UHOL rules}\label{fig:uhol}
\end{figure*}
\end{toappendix}

\subsection{RHOL}

RHOL has non-monadic judgments of the form
$\jrhol{\Gamma}{\Psi}{t_1}{\sigma_1}{t_2}{\sigma_2}{\phi}$, that
combine two typing judgments $\Gamma \vdash t_1 : \sigma_1$,
$\Gamma \vdash t_2 : \sigma_2$, and a logical judgment
$\jhol{\Gamma}{\Psi}{\phi[t_1/\resl][t_2/\resr]}$, where the
distinguished variables $\resl,\resr$ may appear free in
$\phi$ to denote $t_1,t_2$ respectively. 
%A selection of RHOL rules appears in Figure~\ref{fig:rhol}.
The rules
of UHOL are directed by the syntax of $t_1$ and $t_2$, and
we distinguish between
two-sided rules (when both $t_1$ and $t_2$ have the same
top-level type former) and one-sided rules (when we only
look at the top-level type former of one of the two terms).



%\begin{figure*}
%\small
%\begin{gather*}
%\inferrule*[right= \sf ABS]
%      {\jrhol{\Gamma,x_1:\tau_1,x_2:\tau_2}{\Psi,\phi'}{t_1}{\sigma_1}{t_2}{\sigma_2}{\phi}}
%{\jrhol{\Gamma}{\Psi}{\lambda x_1:\tau_1. t_1}{\tau_1 \to \sigma_1}{\lambda x_2:\tau_2. t_2}{\tau_2\to \sigma_2}{\forall x_1,x_2. \phi' \Rightarrow \phi\subst{\resl}{\resl\ x_1}\subst{\resr}{\resr\ x_2}}}
%\\
%\inferrule*[right = \sf APP]
%      {
%\jrhol{\Gamma}{\Psi}{t_1}{\tau_1\to \sigma_1}{t_2}{\tau_2\to \sigma_2}{
%          \forall x_1,x_2. \phi'\subst{\resl}{x_1}\subst{\resr}{x_2}\Rightarrow \phi\subst{\resl}{\resl\ x_1}\subst{\resr}{\resr\ x_2}}\\
%\jrhol{\Gamma}{\Psi}{u_1}{\tau_1}{u_2}{\tau_2}{
%          \phi'}
%}
%{\jrhol{\Gamma}{\Psi}{t_1 u_1}{\sigma_1}{t_2 u_2}{\sigma_2}{\phi\subst{x_1}{u_1}\subst{x_2}{u_2}}}
%\\
%\inferrule*[right = \sf VAR]
%      {\jlc{\Gamma}{x_1}{\sigma_1} \\ \jlc{\Gamma}{x_2}{\sigma_2} \\ \jhol{\Gamma}{\Psi}{\phi\subst{\resl}{x_1}\subst{\resr}{x_2}}}
%{\jrhol{\Gamma}{\Psi}{x_1}{\sigma_1}{x_2}{\sigma_2}{\phi}}
%\\
%\inferrule*[right = \sf ABS{-}L]
%      {\jrhol{\Gamma,x_1:\tau_1}{\Psi, \phi'}{t_1}{\sigma_1}{t_2}{\sigma_2}{\phi}}
%{\jrhol{\Gamma}{\Psi}{\lambda x_1:\tau_1. t_1}{\tau_1 \to \sigma_1}{t_2}{\sigma_2}{\forall x_1. \phi' \Rightarrow \phi \subst{\resl}{\resl\ x_1}}}
%\\
%\inferrule*[right = \sf APP{-}L]
%      {\jrhol{\Gamma}{\Psi}{t_1}{\tau_1\to \sigma_1}{u_2}{\sigma_2}{\forall x_1. \phi'\subst{\resl}{x_1} \Rightarrow \phi\subst{\resl}{\resl\ x_1}}\\
%          \juhol{\Gamma}{\Psi}{u_1}{\sigma_1}{\phi'}}
%{\jrhol{\Gamma}{\Psi}{t_1 u_1}{\sigma_1}{u_2}{\sigma_2}{\phi\subst{x_1}{u_1}}}
%\\
%\inferrule*[right = \sf VAR{-}L]
%      {\phi\subst{\resl}{x_1} \in \Psi \\  \resr\not\in\ FV(\phi) \\
%       \jlc{\Gamma}{t_2}{\sigma_2}}
%      {\jrhol{\Gamma}{\Psi}{x_1}{\sigma_1}{t_2}{\sigma_2}{\phi}}
%\end{gather*}
%\caption{Selected RHOL rules}\label{fig:rhol}
%\end{figure*}

%\subsection{Semantics}
%
%Semantics for these base logics can be given by following the ideas of~\cite{SatoABGGH19}.
%To interpret HOL we need a category whose objects we will use to give semantics
%to logical formulas.
%%
%This category is the category $\Predqbs{}$ as presented before.
%$\Predqbs{}$ is Cartesian closed, and the forgetful functor
%$d: \Predqbs{} \to \QBS$ mapping $(\phi,\sigma)$ to $\sigma$ is faithful and preserves the cartesian closed structure strictly.
%%since $\QBS$ is a quasi-topos, we know that $\QBS/\Omega$ is a CCC. We
%%also let $d : \QBS/\Omega \to \QBS$ denote the domain fibration.
%
%%The semantics of a formula $\phi$ in context $\Gamma$ is an object
%%$\sem{\Gamma\vdash\phi}\in\Pred\QBS$ such that $d(\sem{\Gamma\vdash\phi}) =
%%\sem{\Gamma}$.
%The semantics of a formula $\phi$ in context $\Gamma$ is an object
%$(\sem{\Gamma},\semp{\Gamma\vdash\phi})$, where
%the predicate $\semp{\Gamma\vdash\phi}$ is defined in the standard way.
%The soundness statements are:

%\tetsuya{ Insert definitions of the predicate part. }
%Validity of a judgment $\Gamma\mid\Psi \vdash \phi$ corresponds
%to the existence of a morphism $\sem{\Gamma\vdash\bigwedge\Psi} \to \sem{\Gamma\mid\phi}$
%above the identity $id_{\sem{\Gamma}}$, as stated by the soundness theorem:

%Validity of judgment $\Gamma\mid\Psi \vdash \phi$ is defined by 
%$id_{\sem{\Gamma}} \in \Pred\QBS(\sem{\Gamma\vdash\bigwedge\Psi}, \sem{\Gamma\vdash\phi})$.
%More concretely, this is equivalent to $\semp{\Gamma\vdash\bigwedge\Psi} \subseteq \semp{\Gamma\vdash\phi}$.

%\begin{theorem}\label{thm:hol-soundness}
%If a HOL-judgment $\jhol{\Gamma}{\Psi}{\phi}$ is derivable then it is
%valid, that is $id_{\sem{\Gamma}} \in \Predqbs{}(\sem{\Gamma\vdash\bigwedge\Psi}, \sem{\Gamma\vdash\phi})$.
%\end{theorem}
%\begin{proof}
%The proof is done by the induction on the derivation tree of $\Gamma\mid\Psi \vdash \phi$.
%It is almost obvious.
%We see the rules {Ax}, $\Rightarrow_E$ and $\Rightarrow_I$.
%
%(Ax)
%A judgment of the form $\Gamma\mid \Psi,\phi \vdash \phi$ is always valid:
%\[
%\semp{\Gamma\vdash \bigwedge (\Psi, \phi) } = 
%\semp{\Gamma\vdash (\bigwedge \Psi) \land \phi}
%=
%\semp{\Gamma\vdash \bigwedge \Psi} 
%\cap
%\semp{\Gamma\vdash \phi}
%\subseteq \semp{\Gamma\vdash \phi}.
%\]
%
%($\Rightarrow_I$)
%Suppose that the judgment $\jhol{\Gamma}{\Psi, \phi_1}{\phi_2}$ is derivable.
%By induction hypoithesis, it is valid. 
%Then we have $ \semp{\Gamma\vdash\bigwedge \Psi} \cap \semp{\Gamma\vdash\phi_1} \subseteq \semp{\Gamma\vdash \phi_2}$.
%This implies
%\[ \semp{\Gamma\vdash\bigwedge \Psi} \subseteq 
%(|\sem\Gamma| \setminus \semp{\Gamma\vdash\phi_1})  \cup \semp{\Gamma\vdash \phi_2}
%= \semp{\Gamma\vdash \phi_1 \To \phi_2}.
%\] 
%
%($\Rightarrow_E$)
%Suppose that
%the judgments $\jhol{\Gamma}{\Psi}{\phi_1 \To \phi_2}$ and $\jhol{\Gamma}{\Psi}{\phi_1}$ are derivable. By induction hypoithesis, they are valid. 
%We have
%$\semp{\Gamma\vdash\bigwedge \Psi} \subseteq \semp{\Gamma\vdash \phi_1 \To \phi_2} = 
%|\sem\Gamma| \setminus \semp{\Gamma\vdash \phi_1} \cup \semp{\Gamma\vdash \phi_2}
%$ and 
%$\semp{\Gamma\vdash\bigwedge \Psi} \subseteq \semp{\Gamma\vdash \phi_1}$.
%We have 
%\[
%\semp{\Gamma\vdash\bigwedge \Psi} \subseteq
%(|\sem\Gamma| \setminus \semp{\Gamma\vdash \phi_1} \cup \semp{\Gamma\vdash \phi_2}) \cap 
%\semp{\Gamma\vdash \phi_1}
%\subseteq \semp{\Gamma\vdash \phi_2}. 
%\]
%\end{proof}
%
%This intepretation can be easily extended to UHOL and RHOL:

%\begin{theorem}
%Let $\juhol{\Gamma}{\Psi}{t}{\sigma}{\phi}$ be a derivable UHOL judgment.
%Then it is valid, that is, $\langle \mathrm{id}_{\sem\Gamma}, \sem{\Gamma\vdash t : \sigma} \rangle \in \Predqbs{}(\sem{\Gamma \vdash \bigwedge \Psi},\sem{\Gamma,\mathbf{r}\colon\sigma \vdash \phi})$.
%\end{theorem}
%\begin{proof}
%We remark that for every $\Gamma \vdash e \colon \sigma$, 
%\begin{align*}
%\semp{\Gamma \vdash \phi[e / \mathbf{r}]} & = 
%\{ \xi \in \sem\Gamma ~|~ (\xi,\sem{\Gamma \vdash e}(\xi)) \in \semp{\Gamma,\mathbf{r}\colon\sigma \vdash \phi}\}\\
% &=
%\langle \mathrm{id}_{\sem\Gamma}, \sem{\Gamma\vdash e \colon \sigma} \rangle^{-1} (\semp{\Gamma,\mathbf{r}\colon\sigma \vdash \phi})
%\end{align*}
%
%It suffices to show by induction on derivation tree of $\juhol{\Gamma}{\Psi}{t}{\sigma}{\phi}$.
%\[
%\semp{\Gamma \vdash \bigwedge \Psi} \subseteq \langle \mathrm{id}_{\sem\Gamma}, \sem{\Gamma\vdash t : \sigma} \rangle^{-1} (\semp{\Gamma,\mathbf{r}\colon\sigma \vdash \phi}).
%\]
%{(U-VAR)}
%Suppose $\Gamma | \Psi \vdash \phi[x / \mathbf{r}]$ and $\Gamma \vdash x \colon \sigma$.
%We have $\semp{\Gamma \vdash \bigwedge \Psi} \subseteq \semp{\Gamma \vdash \phi[x / \mathbf{r}]}$ by the soundness of HOL. We obtain, the soundness
%\[
%\semp{\Gamma \vdash \bigwedge \Psi}
%\subseteq \semp{\Gamma \vdash \phi[x / \mathbf{r}]}
%=  \langle \mathrm{id}_{\sem\Gamma}, \sem{\Gamma\vdash x : \sigma} \rangle^{-1} (\semp{\Gamma,\mathbf{r}\colon\sigma \vdash \phi}).
%\]
%
%%We want to show 
%%$
%%\semp{\Gamma \vdash \bigwedge \Psi} \subseteq \langle \mathrm{id}_{\sem\Gamma}, %\sem{\Gamma\vdash x \colon \sigma} \rangle^{-1} (\semp{\Gamma,\mathbf{r}\colon\sigma \vdash \phi})
%%$
%
% 
%\end{proof}


%\begin{theorem}
%Let $\jrhol{\Gamma}{\Psi}{t_1}{\sigma_1}{t_2}{\sigma_2}{\phi}$ be a derivable RHOL judgment.
%Then it is valid, that is, 
%\[\langle \mathrm{id}_{\sem\Gamma}, \sem{\Gamma\vdash t_1 : \sigma_1},
%\sem{\Gamma\vdash t_2 : \sigma_2} \rangle \in 
%\Predqbs{}(\sem{\Gamma \vdash \bigwedge \Psi},\sem{\Gamma,\resl,\colon\sigma_1,
%\resr,\colon\sigma_2 \vdash \phi}).\]
%\end{theorem}

%\subsection{UHOL and RHOL}
%
%Starting from this base logic, we develop our unary and binary program logics.
%Our unary program logic has judgment of the form
%$\juhol{\Gamma}{\Psi}{t}{\sigma}{\phi}$, which combines a typing judgment
%$\Gamma\vdash t :\sigma$ and a logical judgment
%$\jhol{\Gamma}{\Psi}{\phi[t/\res]}$. Here, $\res : \sigma$ is a distinguished
%variable that appears free in $\phi$ to denote the value of $t$. A selection of
%UHOL rules appears in Figure~\ref{fig:uhol}.
%
%
%
%\begin{figure*}
%\small
%\begin{gather*}
%\inferrule*[right = \sf U-VAR]
% {\jlc{\Gamma}{x}{\sigma} \\ \jhol{\Gamma}{\Psi}{\phi\subst{\res}{x}}}
% {\juhol{\Gamma}{\Psi}{x}{\sigma}{\phi}}
%\qquad
%\inferrule*[right= \sf U-ABS]
%  {\juhol{\Gamma,x:\tau}{\Psi,\phi'}{t}{\sigma}{\phi}}
%  {\juhol{\Gamma}{\Psi}{\lambda x:\tau. t}{\tau \to \sigma}{\forall x. \phi'
%    \Rightarrow \phi\subst{\res}{\res\ x}}}
%\\
%\inferrule*[right= \sf U-APP]
%      {\juhol{\Gamma}{\Psi}{t}{\tau\to \sigma}{\forall x.
%        \phi'\subst{\res}{x}\Rightarrow\phi\subst{\res}{\res\ x}}\\ \juhol{\Gamma}{\Psi}{u}{\tau}{\phi'}}
%  {\juhol{\Gamma}{\Psi}{t\ u}{\sigma}{\phi\subst{x}{u}}}
%  \\
%\inferrule*[right = \sf U-SUB]
%    {\juhol{\Gamma}{\Psi}{t}{\sigma}{\phi'} \\
%           \jhol{\Gamma}{\Psi}{\phi'\subst{\res}{t} \Rightarrow \phi\subst{\res}{t}}}
%    {\juhol{\Gamma}{\Psi}{t}{\sigma}{\phi}}
%\end{gather*}
%\caption{Selected UHOL rules}\label{fig:uhol}
%\end{figure*}
%
%On the other hand, our relational logic has judgment of the form
%$\jrhol{\Gamma}{\Psi}{t_1}{\sigma_1}{t_2}{\sigma_2}{\phi}$, that
%combine two typing judgments $\Gamma \vdash t_1 : \sigma_1$,
%$\Gamma \vdash t_2 : \sigma_2$, and a logical judgment
%$\jhol{\Gamma}{\Psi}{\phi[t_1/\resl][t_2/\resr]}$, where the
%distinguished variables $\resl,\resr$ may appear free in
%$\phi$ to denote $t_1,t_2$ respectively. A selection of
%RHOL rules appears in Figure~\ref{fig:rhol}. RHOL combines
%two-sided rules (that depend on both of the programs in the
%judgment) and one-sided rules (that depend only on one).
%
%
%
%\begin{figure*}
%\small
%\begin{gather*}
%\inferrule*[right= \sf ABS]
%      {\jrhol{\Gamma,x_1:\tau_1,x_2:\tau_2}{\Psi,\phi'}{t_1}{\sigma_1}{t_2}{\sigma_2}{\phi}}
%{\jrhol{\Gamma}{\Psi}{\lambda x_1:\tau_1. t_1}{\tau_1 \to \sigma_1}{\lambda x_2:\tau_2. t_2}{\tau_2\to \sigma_2}{\forall x_1,x_2. \phi' \Rightarrow \phi\subst{\resl}{\resl\ x_1}\subst{\resr}{\resr\ x_2}}}
%\\
%\inferrule*[right = \sf APP]
%      {
%\jrhol{\Gamma}{\Psi}{t_1}{\tau_1\to \sigma_1}{t_2}{\tau_2\to \sigma_2}{
%          \forall x_1,x_2. \phi'\subst{\resl}{x_1}\subst{\resr}{x_2}\Rightarrow \phi\subst{\resl}{\resl\ x_1}\subst{\resr}{\resr\ x_2}}\\
%\jrhol{\Gamma}{\Psi}{u_1}{\tau_1}{u_2}{\tau_2}{
%          \phi'}
%}
%{\jrhol{\Gamma}{\Psi}{t_1 u_1}{\sigma_1}{t_2 u_2}{\sigma_2}{\phi\subst{x_1}{u_1}\subst{x_2}{u_2}}}
%\\
%\inferrule*[right = \sf VAR]
%      {\jlc{\Gamma}{x_1}{\sigma_1} \\ \jlc{\Gamma}{x_2}{\sigma_2} \\ \jhol{\Gamma}{\Psi}{\phi\subst{\resl}{x_1}\subst{\resr}{x_2}}}
%{\jrhol{\Gamma}{\Psi}{x_1}{\sigma_1}{x_2}{\sigma_2}{\phi}}
%\\
%\inferrule*[right = \sf ABS{-}L]
%      {\jrhol{\Gamma,x_1:\tau_1}{\Psi, \phi'}{t_1}{\sigma_1}{t_2}{\sigma_2}{\phi}}
%{\jrhol{\Gamma}{\Psi}{\lambda x_1:\tau_1. t_1}{\tau_1 \to \sigma_1}{t_2}{\sigma_2}{\forall x_1. \phi' \Rightarrow \phi \subst{\resl}{\resl\ x_1}}}
%\\
%\inferrule*[right = \sf APP{-}L]
%      {\jrhol{\Gamma}{\Psi}{t_1}{\tau_1\to \sigma_1}{u_2}{\sigma_2}{\forall x_1. \phi'\subst{\resl}{x_1} \Rightarrow \phi\subst{\resl}{\resl\ x_1}}\\
%          \juhol{\Gamma}{\Psi}{u_1}{\sigma_1}{\phi'}}
%{\jrhol{\Gamma}{\Psi}{t_1 u_1}{\sigma_1}{u_2}{\sigma_2}{\phi\subst{x_1}{u_1}}}
%\\
%\inferrule*[right = \sf VAR{-}L]
%      {\phi\subst{\resl}{x_1} \in \Psi \\  \resr\not\in\ FV(\phi) \\
%       \jlc{\Gamma}{t_2}{\sigma_2}}
%      {\jrhol{\Gamma}{\Psi}{x_1}{\sigma_1}{t_2}{\sigma_2}{\phi}}
%\end{gather*}
%\caption{Selected RHOL rules}\label{fig:rhol}
%\end{figure*}
%
%\subsection{Monadic logic}
%
%To reason about monadic computations of type $M \to \cP(\sigma\times M)$ we
%introduce new judgments to UHOL and RHOL. The monadic judgments for UHOL
%are of the form:
%\[ \aumj{\Gamma}{\Psi}{P}{t}{\cT{\sigma}}{Q}{\epsilon} \]
%
%We consider two flavours of this logic:
%\begin{itemize}
%    \item A binary one, where $t$ is a monadic computation over type $\sigma$,
%        $\Gamma, \st : M \vdash P$ is a precondition over the initial memory,
%        and $\Gamma, \st : M, \vl : \sigma \vdash Q$ is a postcondition over
%        the final memory and result.
%%
%    
%    \item A quantitative one, for some set $\Omega$ of truth values. Here $t$
%        is a monadic computation over type $\sigma$, 
%        $\Gamma, \st : M \vdash P : \Omega$ is a precondition over the initial
%        memories, and $\Gamma, \st : M, \vl : \sigma \vdash Q : \Omega$ is a
%        postcondition over the final memories and results.
%\end{itemize}
%
%The syntax itself is independent of the flavour of the logic we choose, they
%only differ in their semantics.
%%
%%The distinguished variables $\st, \vl$ refer to the initial or final memory,
%%and the final value respectively.
%%
%The double brace on the postcondition indicates that even if $Q$ is a
%(binary or quantitative) predicate over $M\times\sigma$, in the context of the
%triple it acts as a predicate over $\cP(M\times \sigma)$, and the $\epsilon$ is
%a grading on the predicate. We assume it is a positive real number, but the
%presentation generalizes to any other semiring.
%
%The unit and bind rules for the monadic logic are in Figure~\ref{fig:muhol}.
%In the UNIT rule, we use an embedding $mk_\Omega(-,-)$, which maps an $\Omega-$
%predicate and a boolean predicate into an $\Omega-$predicate.
%%(if $\Omega = \BB$, then
%%the embedding is just the identity, and if $\Omega = \posr$ then
%%$[\phi]_\Omega$ is the indicator fuction that has value 1 when $\phi$ is
%%satisfied and 0 otherwise).
%
%Analogously we consider monadic judgments for RHOL, that take the form:
%\[ \armj{\Gamma}{\Psi}{P}{t_1}{\cT{\sigma_1}}{t_2}{\cT{\sigma_2}}
%{Q}{\epsilon} \]
%where $P$ is either well-formed of has type $\Omega$ 
%in the context $\Gamma, \stl : M, \str : M$, and $Q$ is well-formed or has
%type $\Omega$ in the context $\Gamma, \stl : M, \str : M, \vll : \sigma_1,
%\vlr : \sigma_2$. Here the variables $\stl,\str$ are used to refer to (resp.
%left or right-side) memories, and $\vll, \vlr$ are used to refer to (resp. left
%or right-side) result values. The unit and bind rules for the relational
%monadic judgments are in Figure~\ref{fig:mrhol}.
%
%
%%\begin{figure*}[!htb]
%%\small
%%\begin{gather*}
%%%
%% \inferrule*[right =\sf Unit-U]
%%  {\uj{\Gamma}{\Psi}{t}{\tau}{\phi}}
%%  {\uj{\Gamma}{\Psi}
%%	  {\unit{t}}{\cT(\tau)}
%%  {\aumon{0}{\res}{P}{P \dot\wedge \phi\subst{\res}{\vl}}}}
%%\qquad
%%\\[0.3em]
%%%
%%\inferrule*[right =\sf Bind-U]
%%{\uj{\Gamma}{\Psi}{t}{\cT(\tau)}{\aumon{\epsilon}{r}{P}{Q}} \\
%%\uj{\Gamma, x : \tau}{\Psi}{u}{\cT(\sigma)}{\aumon{\epsilon'}{\res}{Q\subst{\vl}{x}}{R}} \\  x \not\in R }
%%	  {\uj{\Gamma}{\Psi}
%%  {\mlet{x}{t}{u}}{\cT(\sigma)}{\aumon{\epsilon+\epsilon'}{\res}{P}{R}}}
%%\end{gather*}
%%% \vspace{-0.4cm}
%%\caption{Unary monadic rules}\label{fig:muhol}
%%\end{figure*}
%
%\begin{figure*}[!htb]
%\small
%\begin{gather*}
%%
% \inferrule*[right =\sf Unit-U]
%  {\uj{\Gamma}{\Psi}{t}{\tau}{\phi} \\
%  \holwf{\Gamma, \st : M}{P : \Omega}}
%  {\aumj{\Gamma}{\Psi}{P}
%  {\unit{t}}{\cT(\tau)}{mk_\Omega(P,\phi\subst{\res}{\vl})}{0}}
%\qquad
%\\[0.3em]
%%
%\inferrule*[right =\sf Bind-U]
%{\aumj{\Gamma}{\Psi}{P}{t}{\cT(\tau)}{Q}{\epsilon} \\
%\aumj{\Gamma, x : \tau}{\Psi}{Q\subst{\vl}{x}}{u}{\cT(\sigma)}{R}{\epsilon'} \\  x \not\in R }
%{\aumj{\Gamma}{\Psi}{P}
%{\mlet{x}{t}{u}}{\cT(\sigma)}{R}{\epsilon+\epsilon'}}
%\end{gather*}
%% \vspace{-0.4cm}
%\caption{Unary monadic rules}\label{fig:muhol}
%\end{figure*}
%
%
%
%\begin{figure*}[!htb]
%\small
%\begin{gather*}
%%
% \inferrule*[right =\sf Unit]
% {\rj{\Gamma}{\Psi}{t_1}{\tau_1}{t_2}{\tau_2}{\phi} \\
%  \holwf{\Gamma, \stl: M, \str : M}{P}}
% {\armj{\Gamma}{\Psi}{P}
%	  {\unit{t_1}}{\cT(\tau_1)}{\unit{t_2}}{\cT(\tau_2)}
%  {mk_\Omega(P,\phi)}{0}}
%\qquad
%\\[0.3em]
%%
%\inferrule*[right =\sf Bind]
%{\armj{\Gamma}{\Psi}{P}{t_1}{\cT(\tau_1)}{t_2}{\cT(\tau_2)}{Q}{\epsilon} \\
%	\armj{\Gamma, x_1 : \tau_1, x_2 : \tau_2}{\Psi}{Q\subst{\vll}{x_1}\subst{\vlr}{x_2}}
%{u_1}{\cT(\sigma_1)}{u_2}{\cT(\sigma_2)}{R}{\epsilon'} \\  x_1,x_2 \not\in R }
%{\armj{\Gamma}{\Psi}{P}
%{\mlet{x_1}{t_1}{u_1}}{\cT(\sigma_1)}{\mlet{x_2}{t_2}{u_2}}{\cT(\sigma_2)}{R}{\epsilon+\epsilon'}}
%\end{gather*}
%% \vspace{-0.4cm}
%\caption{Relational monadic rules}\label{fig:mrhol}
%\end{figure*}
%
%Apart from the standard monadic constructions of unit and binding, which have
%generic rules, we need to provide rules for the monadic operations of our
%language: reading, writing and sampling. These however, need concrete rules
%for each of the instantiations of the logic we may consider.
%In Figure~\ref{fig:u-mon-op} we provide the rules for the particular case
%of a unary logic with boolean-valued predicates, and concretely for
%uniform sampling from a finite domain.
%We will later present rules for other logics and other probability
%distributions after introducing other instantiations of our framework.
%
%\begin{figure*}[!htb]
%\small
%\begin{gather*}
%%
% \inferrule*[right =\sf Sample-U]
% { |\{x\in \sigma \mid x \in \phi \}|\,/\,|\sigma|\, =\, \delta  }
%  {\aumj{\Gamma}{\Psi}{P}
%  {\unif{\sigma}}{\cT(\tau)}{P\wedge \phi}{1-\delta}}
%\qquad
%\\[0.3em]
%%
%\inferrule*[right =\sf Read-U]
%{\uj{\Xi;\Gamma}{\Psi}{a}{\loc}{\psi}\\
%\jhol{\Gamma}{\Psi}{\forall m, l. P(m) \Rightarrow \psi(l) \Rightarrow \phi(h(l))}}
%{\aumj{\Gamma}{\Psi}{P}
%{\rd{a}}{\cT(\tval)}{P \wedge \phi}{1}}
%\\[0.3em]
%\inferrule*[right =\sf Write-U]
%{\Xi;\Gamma \vdash a : \loc \\
% \Xi;\Gamma \vdash t : \tval  }
%{\aumj{\Gamma}{\Psi}{P\subst{s}{s[a\mapsto t]}}
%{\wrt{a}{t}}{\cT(\tunit)}{P}{1}}
%\end{gather*}
%% \vspace{-0.4cm}
%\caption{Unary rules for monadic operations}\label{fig:u-mon-op}
%\end{figure*}

